Evaluating Design Tradeoffs in Numeric Static Analysis for Java

Numeric static analysis for Java has a broad range of potentially useful applications, including array bounds checking and resource usage estimation. However, designing a scalable numeric static analysis for real-world Java programs presents a multitude of design choices, each of which may interact with others. For example, an analysis could handle method calls via either a top-down or bottom-up interprocedural analysis. Moreover, this choice could interact with how we choose to represent aliasing in the heap and/or whether we use a relational numeric domain, e.g., convex polyhedra. In this paper, we present a family of abstract interpretation-based numeric static analyses for Java and systematically evaluate the impact of 162 analysis configurations on the DaCapo benchmark suite. Our experiment considered the precision and performance of the analyses for discharging array bounds checks. We found that top-down analysis is generally a better choice than bottom-up analysis, and that using access paths to describe heap objects is better than using summary objects corresponding to points-to analysis locations. Moreover, these two choices are the most significant, while choices about the numeric domain, representation of abstract objects, and context-sensitivity make much less difference to the precision/performance tradeoff.

==> Makefile <==
OS   := $(shell uname)
ifeq ($(OS), Linux)
  OPEN := evince
else
  OPEN := open -a /Applications/Skim.app
endif
DOC  := doc-pldi2017
MAIN := paper
PDFLATEX := pdflatex

DEP := *.tex *.bib
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))

start:
	make open
	make watch

open: $(DOC).pdf
	@$(OPEN) $<

$(DOC).pdf: $(DEP)
	perl watch.pl render_latex $(MAIN) "\input{$(MAIN).tex}"
	@cp $(MAIN).pdf $(DOC).pdf
	@cp $(MAIN).synctex.gz $(DOC).synctex.gz
watch:
	perl watch.pl watch $(DOC).pdf $(DEP)

debug: $(DEP)
	$(PDFLATEX) -interaction nonstopmode "\input{$(MAIN).tex}"
	$(OPEN) $(DOC).pdf

clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.run.xml; true
	rm -Rf *~; true
	rm -Rf $(DOC).pdf $(MAIN).pdf; true
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true

desvn:
	find . -type d -name .svn -exec rm -rf {} +


==> old-introNperf.tex <==
\section{Old Introduction}

The abstract interpretation~\cite{Cousot:1977:AIU:512950.512973}
community has developed a wide variety of techniques to support static
analysis of numeric program properties (``numeric static analysis'').
Such analyses can detect buffer overflows~\cite{wagner:ndss00}, analyze a program's resource
usage~\cite{Gulwani:2010:RP:1806596.1806630,Gulwani:2009:CRP:1542476.1542518},
detect side
channels~\cite{Brumley:2003:RTA:1251353.1251354,Bortz:2007:EPI:1242572.1242656},
and discover vectors for denial of service
attacks~\cite{hashtable-attack,hash-dos}.

We aim to apply fully automatic, numeric static analysis to real-world software written
in Java. The basic approach is clear: we need to combine some numeric
domain with a model of the heap, and we need to account for method
calls (i.e., make the analysis
interprocedural). Fu~\cite{fu2014modularly} and Ferrara et
al~\cite{ferrara2014generic,ferrara2015automatic} show how to combine
a heap analysis (such as a points-to
analysis~\cite{Landi:1992:SAA:143095.143137} or shape
analysis~\cite{Sagiv:1999:PSA:292540.292552}) with a numeric domain
(such as intervals or polyhedra~\cite{Cousot:1977:AIU:512950.512973}).
But they stop short of exploring the needed ingredients for a scalable
tool. For example, neither consider method
calls: Fu ignores the effect of calls, making unsound
assumptions about heap-allocated objects, while Ferrara et al. focus on
inferring challenging invariants in small, non method-calling
programs. Clousot~\cite{logozzoclousot} checks numeric assertions on
heap-manipulating, interprocedural programs, but to do so must make
strong assumptions about (non)aliasing of method arguments, and
expects programmers to specify method pre- and post-conditions.
(Section~\ref{sec:related} considers related work in
detail.) Beyond the handling of method calls, there are a multitude of
other design choices in scaling abstract interpretation to large Java
programs. But these have not been evaluated systematically in the
literature, so we were left to wonder: how do various
choices trade precision and performance?

In this paper, we develop a family of combined numeric and heap
analyses for Java. We use multiple linear regression to determine how
design choices affect performance, precision, and the tradeoff between
the two, considering a total of \mwh{216?} variations.
As far as we are aware, our basic analysis is one of the few
combined numeric and heap analyses that is fully automated and scales
to large Java programs. We do not know of any prior work that has considered so many
analysis variations simultaneously.

Our analyses use a combination of numeric domains, a
points-to analysis for the heap, and heap-based strong updates. In more
detail, the analyses employ an ahead-of-time points-to 
analysis~\cite{Smaragdakis:2015:PA:2802194.2802195} to name locations
in the heap. The analysis can then associate standard numeric domains
(such as intervals) with both local and heap-allocated objects. To
improve precision, we allow strong
updates~\cite{Chase:1990:APS:93542.93585} on heap-allocated data by
separately tracking numeric values named by \emph{access
  paths}~\cite{De:2012:SFP:2367163.2367203,Wei:2014:SPA:2945642.2945644}. For example, if \code{a1} and \code{a2} may alias
according to the points-to analysis, then after a write \code{a2.f =
  42} our analysis strongly updates the value for access path
\code{a2.f} to be \code{42}. Thus, if \code{a2.f} is subsequently
accessed before either \code{a1} or \code{a2} is written, the analysis
still knows the precise value of
\code{a2.f}. \mwh{new stuff: inlining, special handling of access paths}
(Section~\ref{sec:analysis} describes our basic combined
numeric and heap analysis in detail.)

\mwh{Lots of what follows will need to be updated.}
We construct a family of 
interprocedural analyses by varying five
options. The first option is the analysis direction, which is either
\emph{top-down} (TD) or \emph{bottom-up} (BU), i.e., it either
proceeds from the \code{main} method forward through the program, or
it starts at leaf methods and works its way backward,
respectively. TD analysis is simple and precise, but it may analyze the
same method multiple times in different contexts. In contrast, a
BU analysis is expensive for each individual method, but that
method will only be analyzed once and its summary used at any call
sites, which may be a better tradeoff. As mentioned earlier, the most
related prior work ignores interprocedural
analysis entirely, so our overall (numeric+heap+methods) analysis is novel. The TD
analysis is straightforward, but the BU analysis requires more careful
handling of heap-allocated objects, constituting an interesting
contribution in its own right. \jeff{Describe idea of previous.}
(Section~\ref{app:interproc} describes the top-down and bottom-up
approaches.)

The other four options we vary are more standard. We vary the \emph{numeric
domain} (interval, polyhedral, or a combination of them via
``packing'' \cite{cousot2005astree}, considering both block-level
and method-level packs); \emph{context-sensitivity} of the points-to analysis
(context-insensitive, 1-CFA~\cite{shivers91}, or type-sensitivity
\cite{smaragdakis2011pick}); the \emph{object representation} (class-based,
allocation-site based, or allocation-site based except for strings);
and \emph{widening} (done after either one, three, or 10
iterations)\pxm{The widening variations ended up not mattering,
  perhaps this could be removed from experiments?}.
(Section \ref{sec:custom} describes these analysis variants.) Our
implementation uses
WALA~\cite{wala} and
PPL~\cite{Bagnara:2008:PPL:1385689.1385711} (Section \ref{sec:impl}).

Finally, we apply all of 216 analysis variants to five\pxm{all Java
  programs from the ...?} Java programs
from the DaCapo benchmark suite~\cite{DaCapo:paper}. To measure
precision, we used the results of the analysis for two clients:
checking array indexes are in bounds and estimating values of
numerically-typed fields. The latter is particularly useful as a
comparison point for analyses that ignore the heap entirely; doing so
soundly would mean all fields could take any value.
We measured the analysis running time, and
the precision of each client in terms of the number of
array accesses provably in bounds and the count of unconstrained field reads.
We define the tradeoff of the two as the precision divided by the
performance, i.e., the number of checks discharged per minute of
analysis time.  We then performed multiple linear regression to
determine how analysis options affected performance, precision, and
the tradeoff.

We observed several interesting results. First, as expected,
polyhedra are far more precise than intervals, but can be orders of
magnitude more expensive. Fortunately, using method-level packing
loses little in terms of precision and gains much in
performance. Second, BU analysis is generally faster, but requires
using a (partially) relational domain to be competitive with TD in
terms of precision. This makes sense: BU summaries of methods are most
useful when they can relate inputs to outputs and/or side effects on
the heap. Third, context-sensitive points-to information does not 
benefit our analysis. This is because standard numeric abstract
interpretation is already flow- and context-sensitive,
i.e., it treats each call to a method distinctly from other calls.
The loss of context-sensitive aliasing information when analyzing a
called method seems not to harm precision. Finally, an allocation
site-based object representation but with special
handling of strings provided the best tradeoff generally, but not
as significantly in the BU case. Section~\ref{sec:eval}
provides details and additional observations. 


\section{Old Evaluation}
\subsection{RQ1: Performance}
\label{acimpact}

\begin{table}[t!]
%\nocaptionrule
\small
\centering
\begin{tabular}{|c|c|r|r|r|}
\hline
{\bf Option} & {\bf Setting} & \parbox{0.3in}{\centering \bf Est. (min)} & \multicolumn{1}{c|}{\bf CI} & {\bf $p$-value} \\
\hline \hline
\multirow{2}{*}{\opt{AO}} & \opt{TD} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU} &  \cellcolor{green}-25.4 & \cellcolor{green}[-39.0, -11.8] & \cellcolor{green}$<$0.001 \\
\hline
\multirow{4}{*}{\opt{DP}} & \opt{INT} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{POL} &  \cellcolor{green}127.1 & \cellcolor{green}[113.5, 140.7] & \cellcolor{green} $<$0.001 \\
\hhline{~----}
 & \opt{HY1} & 0.1 & [-13.5, 13.7] & 0.987\\
\hhline{~----}
 & \opt{HY2} & 13.5 & [-0.1,  27.1] & 0.051\\
 \hline
 \multirow{3}{*}{\opt{CS}} & \opt{CI} & - & - & - \\
\hhline{~----}
 & \opt{1CFA} & 11.6 & [-0.19,  23.4] & 0.053 \\
\hhline{~----}
 & \opt{1TYP} & 3.7 & [-8.1,  15.5] & 0.539 \\
 \hline
\multirow{3}{*}{\opt{OR}} & \opt{CLAS} & - & - & - \\
\hhline{~----}
 & \opt{SMUS} & -7.8 & [-23.4, 7.7] & 0.324 \\
\hhline{~----}
 & \opt{ALLO} & -9.2 &  [-24.7, 6.4] & 0.248 \\
 \hline
 \multirow{3}{*}{\opt{WI}} & \opt{W1} & - & - & - \\
\hhline{~----}
 & \opt{W3} & 0.2 & [-5.7, 6.1] & 0.946 \\
\hhline{~----}
 &\cellcolor{green}\opt{W10} &  \cellcolor{green}15.3 & \cellcolor{green}[9.4, 21.2] & \cellcolor{green}$<$0.001 \\
 \hline
 \hline
  \multirow{4}{*}{\opt{AO:DP}} & \opt{TD:INT} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:POL} & \cellcolor{green}-73.8 & \cellcolor{green}[-87.3, -60.2] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \opt{BU:HY1} & -0.2 & [-13.5, 13.7] & 0.977 \\
\hhline{~----}
 & \opt{BU:HY2} & -1.0 & [-14.6, 12.6] & 0.882 \\
 \hline
 \multirow{3}{*}{\opt{AO:CS}} & \opt{TD:CI} & - & - & - \\
\hhline{~----}
 & \opt{BU:1CFA} & -0.3 &  [-12.1, 11.5] & 0.960 \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:1TYP} & \cellcolor{green}32.1 & \cellcolor{green}[20.4, 43.9] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{3}{*}{\opt{AO:OR}} & \opt{TD:CLAS} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:SMUS} & \cellcolor{green}23.9 & \cellcolor{green}[12.1, 35.7] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:ALLO} & \cellcolor{green}82.0 & \cellcolor{green}[70.2, 93.7] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{7}{*}{\opt{DP:OR}} & \opt{INT:CLAS} & -  & - & - \\
\hhline{~----}
 & \opt{POL:SMUS} & -8.2 &  [-24.9, 8.4] & 0.331 \\
\hhline{~----}
 & \cellcolor{green}\opt{POL:ALLO} & \cellcolor{green}-18.5 & \cellcolor{green}[-35.2, -1.9] & \cellcolor{green}0.029 \\
\hhline{~----}
 & \opt{HY1:SMUS} & 0.4 &  [-16.3, 17.0] & 0.966 \\
\hhline{~----}
 & \opt{HY1:ALLO} & 1.9 & [-14.7, 18.6] & 0.822 \\
\hhline{~----}
 & \opt{HY2:SMUS} & 14.5 & [-2.1, 31.2] & 0.086 \\
\hhline{~----}
 & \opt{HY2:ALLO} & 9.6 & [-7.0, 26.3] & 0.258 \\
 \hline
 \multirow{5}{*}{\opt{CS:OR}} & \opt{CI:CLAS} & - & - & - \\
\hhline{~----}
 & \opt{1CFA:SMUS} & -6.2 &  [-20.6, 8.2] & 0.398 \\
\hhline{~----}
 & \opt{1TYP:SMUS} & 0.4 & [-14.0, 14.9] & 0.952 \\
\hhline{~----}
 & \cellcolor{green}\opt{1CFA:ALLO} & \cellcolor{green}-24.9 & \cellcolor{green}[-39.4, -10.5] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
  & \cellcolor{green}\opt{1TYP:ALLO} & \cellcolor{green}28.8 & \cellcolor{green}[14.4, 43.2] & \cellcolor{green}$<$0.001 \\
 \hline
\end{tabular}
\caption{\textmd{Performance over all benchmark programs. Lower is better in Est. column. R$^2$ of 0.65.}}
\vspace{1pt}
\hrule
\vspace{-12pt}
\label{table:performance}
%\jeff{Indicate in caption whether positive or negative values are good.}
\end{table}

Table \ref{table:performance} presents a summary of a regression
that shows the effect of analysis configuration options on
performance. We measure performance as the time to run the core
analysis and then use the results to implement the checks for \aarray{}
and \afield{}.
% \footnote{We also include a third client that counts non-$\top$
%   return values; we do not discuss that client due to lack of space,
%   but the added time for it is negligible. \jeff{I assume this is not
%    included in the new numbers?}}
 In the top part of the figure, the first column shows the
independent variables and the second column shows a setting. One of
the settings, identified by dashes in the remaining columns, is the
baseline in the regression. (The baseline configuration in
Table~\ref{table:benchmarks} is the combination of these baseline settings). For the other
settings, the third column shows the estimated effect of that setting
with all other settings (including the choice of program) held fixed.
For example,
the second row of the table shows that bottom-up analysis decreases
overall analysis time by 25.4 minutes compared to top-down
analysis, using the baseline settings of the other options. 
\jeff{Is that on average across programs?}
The fourth column shows
the 95\% confidence interval around the
estimate, and the last column shows the $p$-value. As is standard, we
consider $p$-values less than 0.05 (5\%) significant; such rows are
highlighted in green in the table. \jeff{What happens if the analysis
  didn't complete? We mention this in the next two sections but not here.}

The bottom part of the table is similar, but it shows the additional effects of
two-way combinations of options compared to the baseline effects of
each option. For example, the \opt{BU:POL} line shows that bottom-up,
polyhedral analysis is 27.9 minutes slower compared to the effect of
top-down, interval analysis (\opt{TD:INT}). We count this effect by adding the
individual effects of \opt{BU} (-25.4) and \opt{POL} (127.1) as
well as the \opt{BU:POL} interaction (-73.8). Note that
not all interactions are shown (e.g., \opt{AO:WI} is not in the table). Any
interactions not included were found, during model generation, to be
unnecessary to explain difference from the baseline, i.e., they have
no meaningful effect.

Note that although we included the program as an independent variable
in the regression, we do not discuss the effect of particular programs
here. As mentioned above, including the program as a variable allows
us factor out program-specific influence and thus focus on the general
effect of the analysis options. \jeff{This sounds wishy-washy. Can we
  be more precise? Some readers will wonder why we don't normalize, so
we should explain exactly what we're measuring by including the
programs as a variable.}

We observe several interesting results from Table \ref{table:performance}.

\emph{Using polyhedra incurs significant slowdown though not as much
  with bottom-up analysis.} Overall, polyhedral analysis (\opt{POL})
is two hours slower than using the interval domain, which is a large
effect with high significance. Indeed, 137 out of 205 analyses that
timed out used the polyhedral domain. However, when we combine bottom-up
analysis with polyhedra (\opt{BU:POL}), the slowdown relative to \opt{TD:INT}
is only 25 minutes (as calculated above). This trend matches our timeout data:
68\% (i.e., 93 out of 137) analyses that
timed out using polyhedra are also top-down.

\emph{Bottom-up analysis is faster than top-down analysis in general,
  but is more sensitive to other options.} We see that bottom-up
analysis (\opt{BU}) has an overall benefit of $25.4$ minutes by itself,
compared to top-down analysis.  However, when combined with
allocation-based object representation, bottom-up analysis is
$56.6$ minutes slower than a top-down
analysis (i.e., the individual effect of \opt{BU}, $-25.4$,
plus the \opt{BU:ALLO} interaction, $82.0$). We believe this is because
our bottom-up analysis introduces 
``initial paths" for each heap object access
(Section \ref{ana:bu}). These additional
abstract objects in the numeric domain slow down the
analysis relative to a top-down approach. This is especially
pronounced for string-manipulating functions---\opt{BU:SMUS} offers
considerably less slowdown. \opt{BU:1TYP} also incurs a significant
additional slow-down.

\emph{Context-sensitivity interacts with object-representation, and
  more aggressive widening improves performance.} We see that
combining allocation-site object-representation with 1-CFA
(\opt{1CFA:ALLO}) and combining it with type-sensitive analysis
(\opt{1TYP:ALLOC}) have approximately equal and opposite
effects. In other words, type-sensitive analysis is more efficient
with class-based object representation and 1-CFA analysis is more
efficient with allocation-based representation. This may be related to
the design of type-sensitive analysis, which uses the class names of
the receiver objects as calling contexts. We also see that widening
more aggressively
(after one or three iterations) is faster than widening after 10
iterations (\opt{W10}).

\subsection{RQ2: Precision}
\label{sec:precision}

\begin{table}[t]
%\nocaptionrule
\small
\centering
\begin{tabular}{|c|c|r|r|r|}
\hline
{\bf Option} & {\bf Setting} & \textbf{Est. (\#)} & \multicolumn{1}{c|}{\bf CI} & {\bf $p$-value} \\
\hline \hline
\multirow{2}{*}{\opt{AO}} & \opt{TD} & -& - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU} & \cellcolor{green}-38.8 & \cellcolor{green}[-44.1, -33.5] & \cellcolor{green}$<$0.001 \\
\hline
\multirow{4}{*}{\opt{DP}} & \opt{INT} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{POL} & \cellcolor{green}30.0 & \cellcolor{green}[23.4, 36.6] & \cellcolor{green} $<$0.001 \\
\hhline{~----}
 & \opt{HY1} & 4.3 & [-0.4, 9.1] & 0.071\\
\hhline{~----}
 & \cellcolor{green}\opt{HY2} & \cellcolor{green}26.2 & \cellcolor{green}[21.3, 31.08] & \cellcolor{green}$<$0.001 \\
 \hline
\multirow{3}{*}{\opt{OR}} & \opt{CLAS} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{SMUS} & \cellcolor{green}7.2 & \cellcolor{green}[2.7, 11.7] & \cellcolor{green}0.002 \\
\hhline{~----}
 & \cellcolor{green}\opt{ALLO} & \cellcolor{green}11.1 & \cellcolor{green}[6.6, 15.7] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{2}{*}{\opt{CL}} & \opt{FD} & -& - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{AR} & \cellcolor{green}-51.7 & \cellcolor{green}[-57.0, -46.3] & \cellcolor{green}$<$0.001 \\
\hline
 \hline
  \multirow{4}{*}{\opt{AO:DP}} & \opt{TD:INT} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:POL} & \cellcolor{green}40.3 & \cellcolor{green}[33.2, 47.4] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \opt{BU:HY1} & -1.8 & [-7.4, 3.7] & 0.518 \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:HY2} & \cellcolor{green}41.2 & \cellcolor{green}[35.5, 47.0] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{3}{*}{\opt{AO:OR}} & \opt{TD:CLAS} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:SMUS} & \cellcolor{green}-12.3 & \cellcolor{green}[-17.4, -7.2] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:ALLO} & \cellcolor{green}-13.1 & \cellcolor{green}[-18.5, -7.8] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{2}{*}{\opt{AO:CL}} & \opt{TD:FD} & -& - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{BU:AR} & \cellcolor{green}27.5 & \cellcolor{green}[23.2, 31.8] & \cellcolor{green}$<$0.001 \\
\hline
\multirow{4}{*}{\opt{DP:CL}} & \opt{INT:FD} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{POL:AR} & \cellcolor{green}-26.3 & \cellcolor{green}[-33.0, -19.5] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \opt{HY1:AR} & -3.1 & [-8.7, 2.4] & 0.267 \\
\hhline{~----}
 & \cellcolor{green}\opt{HY2:AR} & \cellcolor{green}-25.6 & \cellcolor{green}[-31.3, -19.9] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{3}{*}{\opt{OR:CL}} & \opt{CLAS:FD} & - & - & - \\
\hhline{~----}
 & \cellcolor{green}\opt{SMUS:AR} & \cellcolor{green}144.3 & \cellcolor{green}[139.2, 149.3] & \cellcolor{green}$<$0.001 \\
\hhline{~----}
 & \cellcolor{green}\opt{ALLO:AR} & \cellcolor{green}147.7 & \cellcolor{green}[142.4, 153.0] & \cellcolor{green}$<$0.001 \\
 \hline
\end{tabular}
%\jeff{Indicate in caption whether positive or negative values are good.}
\caption{\textmd{Precision for \aarray{} (\opt{AR}) and \afield{} (\opt{FD}). Positive values
    in Est. column indicate better precision. R$^2$ of 0.96.}}
\hrule
\vspace{-12pt}
\label{tab:precision}
\end{table}

Table~\ref{tab:precision} summarizes a regression showing how option
settings affect precision. As before, we include the benchmark program as an
independent variable, but we omit its effects from the table.
We also add the analysis client---option \opt{CL} with
settings \opt{FD} for \afield{} and \opt{AR} for \aarray{}---as an
independent variable so we can analyze differences
between the analyses. 
 The dependent variable is the number of checks
discharged by the analysis.  Thus, in absolute terms, the analyses can
discharge 51.7 fewer checks for \aarray{} than for \afield{} (line
\opt{AR} in the table). Statistically significant settings and
interactions are highlighted in green.  If an analysis did not complete under a given
configuration, we omit those configurations from the
regression.

We see several interesting results
from Table \ref{tab:precision}.

\emph{More relational domains improves precision, especially for \afield{}.} 
Using polyhedra (\opt{POL}) or method-level packing (\opt{HY2}) 
improve precision by about 30 more checks. However, the \opt{POL:AR}
and \opt{HY2:AR} interactions also 
show that the more precise numeric domains are less important to the
precision of \aarray{}, likely because the precision of
\aarray{} is dominated by object representation, as discussed just above.

\emph{The bottom-up analysis harms precision overall, but is boosted
  by relational domains.} In general, bottom-up analysis (\opt{BU})
has a negative effect on precision (38.8 fewer checks)
compared to top-down. However, when combined with
\opt{POL} or \opt{HY2}, precision of \opt{BU} matches that of
\opt{TD}. For example, \opt{POL} adds 30.0; while
\opt{BU} subtracts 38.8 from this it adds 40.3
for \opt{BU:POL}. Interaction \opt{BU:HY2} compensates similarly. This
makes sense because \opt{BU} method summaries work best when they
relate a method's inputs to its effects and outputs, and such
relations cannot be captured by \opt{INT}.
  
\emph{Widening and context-sensitivity are not significant.} 
Widening and context-sensitivity do not appear in the model, meaning
they do not affect precision significantly. 
This makes sense because both the \opt{TD} and \opt{BU} analyses are
already somewhat context-sensitive when run with the \opt{CI} option. 
\jeff{This should be mentioned earlier in the paper, and there should
  be a back reference here to that discussion.}
For \opt{TD} each call will be interpreted in the context of the
current abstraction, and for \opt{BU} it will be instantiated in it;
only aliasing constraints will be context-insensitive. 
For widening, the likely explanation is the lack of loops that run for
a fixed number of iterations that is less than 3, or 10, for which no
loss of precision due to widening is incurred. 

\emph{More precise object representation improves precision,
  especially for \opt{TD} \aarray{}.} 
Strong \opt{SMUS:AR}
and \opt{ALLO:AR} interactions show that object representation is the
most dominant factor in the precision of \aarray{} (the added $144+$
checks easily overcoming the relatively fewer number of \opt{AR}
checks, $-51.7$, compared to \opt{FD}). 
With top-down they do even better (\opt{SMUS} and \opt{ALLO} add 7.2
and 11.1, resp.), while for \opt{BU} they do slightly worse.  Array
checking using \opt{CLAS} does worse because it conflates all arrays
of the same type as one abstract object, thus imprecisely
approximating those arrays' lengths, causing some checks to spuriously
fail.

\subsection{RQ3: Tradeoffs}
\begin{table*}[t]
%\nocaptionrule
\small
\centering
% Central table.
\begin{tabular}{l l}
  % Left hand side of the table.
  \begin{tabular}{|c|c|r|r|r|}
    \hline
  {\bf Option} & {\bf Setting} & \textbf{Est. (\#)} & \multicolumn{1}{c|}{\bf CI} & {\bf $p$-value} \\
    \hline
    \multirow{2}{*}{\opt{AO}} & \opt{TD} & -& - & - \\
    \hhline{~----}
     & \cellcolor{green}\opt{BU} & \cellcolor{green}28.3583 & \cellcolor{green}[23.3, 47.2] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{4}{*}{\opt{DP}} & \opt{INT} & - & - & - \\
    \hhline{~----}
    & \opt{HY1} & -2.1396 & [-9.7,5.4] & 0.579 \\
    \hhline{~----}
    & \cellcolor{green}\opt{HY2} & \cellcolor{green}-24.3592 & \cellcolor{green}[-31.9,-16.7] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{POL} & \cellcolor{green}-48.6091 & \cellcolor{green}[-56.1,-41.0] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{3}{*}{\opt{CS}} & \opt{CI} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{1CFA} & \cellcolor{green}-17.6066 & \cellcolor{green}[-24.5,-10.6] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1TYP} & \cellcolor{green}-32.6407 & \cellcolor{green}[-39.5,-25.7] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{3}{*}{\opt{OR}} & \opt{CLAS} & - & - & - \\
    \hhline{~----}
    & \opt{ALLO} & 0.4072 & [-6.5,7.3] & 0.908 \\
    \hhline{~----}
    & \cellcolor{green}\opt{SMUS} & \cellcolor{green}12.9499 & \cellcolor{green}[6.0,19.8] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{3}{*}{\opt{WI}} & \opt{W1} & - & - & - \\
    \hhline{~----}
    & \opt{W3} & -2.9252 & [-9.4,3.6] & 0.382 \\
    \hhline{~----}
    & \cellcolor{green}\opt{W10} & \cellcolor{green}-33.8812 & \cellcolor{green}[-40.4,-27.3] & \cellcolor{green}$<$0.001 \\
    \hline
    
    \multirow{2}{*}{\opt{CL}} & \opt{FD} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{AR} & \cellcolor{green}7.6265 & \cellcolor{green}[1.9,13.2] & \cellcolor{green}0.008 \\
    \hline

    \multirow{4}{*}{\opt{AO:DP}} & \opt{TD:INT} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:HY1} & \cellcolor{green}5.4758 & \cellcolor{green}[0.4,10.5] & \cellcolor{green}0.033 \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:HY2} & \cellcolor{green}10.5236 & \cellcolor{green}[5.4,15.5] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:POL} & \cellcolor{green}17.7632 & \cellcolor{green}[12.7,22.8] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{7}{*}{\opt{DP:CS}} & \opt{INT:CI} & - & - & - \\
    \hhline{~----}
    & \opt{HY1:1CFA} & 0.5547 & [-5.6, 6.7] & 0.860 \\
    \hhline{~----}
    & \cellcolor{green}\opt{HY2:1CFA} & \cellcolor{green}7.9726 & \cellcolor{green}[1.7, 14.1] & \cellcolor{green}0.011 \\
     \hhline{~----}
    & \opt{POL:1CFA} & 4.5400 & [-1.6, 10.7] & 0.150 \\
     \hhline{~----}
    & \opt{HY1:1TYP} & 2.3923 & [-3.7, 8.5] & 0.448 \\
     \hhline{~----}
     & \cellcolor{green}\opt{HY2:1TYP} & \cellcolor{green}14.7121 & \cellcolor{green}[8.5, 20.8] & \cellcolor{green}$<$0.001 \\
     \hhline{~----}
     & \cellcolor{green}\opt{POL:1TYP} & \cellcolor{green}22.3021 & \cellcolor{green}[16.1, 28.4] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{7}{*}{\opt{DP:OR}} & \opt{INT:CLAS} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{HY1:ALLO} & \cellcolor{green}-7.593 & \cellcolor{green}[-13.7, -1.4] & \cellcolor{green}0.016 \\
    \hhline{~----}
    & \opt{HY2:ALLO} & -5.2126 & [-11.3, 0.9] & 0.098 \\
     \hhline{~----}
    & \opt{POL:ALLO} & -0.7067 & [-6.8, 5.4] & 0.822 \\
     \hhline{~----}
    & \opt{HY1:SMUS} & -4.4587 & [-10.6, 1.7] & 0.157 \\
     \hhline{~----}
     & \cellcolor{green}\opt{HY2:SMUS} & \cellcolor{green}-11.7440 & \cellcolor{green}[-17.9, -5.5] & \cellcolor{green}$<$0.001 \\
     \hhline{~----}
     & \cellcolor{green}\opt{POL:SMUS} & \cellcolor{green}-7.4024 & \cellcolor{green}[-13.5, -1.2] & \cellcolor{green}0.019 \\
    \hline

    \multirow{3}{*}{\opt{AO:CS}} & \opt{TD:CS} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:1CFA} & \cellcolor{green}-21.2563 & \cellcolor{green}[-25.6,-16.8] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:1TYP} & \cellcolor{green}-25.5611 & \cellcolor{green}[-29.9,-21.1] & \cellcolor{green}$<$0.001 \\
    \hline
 
  \end{tabular}

  % Right hand side of the table.
  \begin{tabular}{|c|c|r|r|r|}
    \hline
  {\bf Option} & {\bf Setting} & \textbf{Est. (\#)} & \multicolumn{1}{c|}{\bf CI} & {\bf $p$-value} \\
    \hline

    \multirow{3}{*}{\opt{AO:OR}} & \opt{TD:CLAS} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{BU:ALLO} & \cellcolor{green}-52.5418 & \cellcolor{green}[-56.9,-48.1] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \opt{BU:SMUS} & -3.2799 & [-7.6,1.0] & 0.141 \\
    \hline

    \multirow{7}{*}{\opt{DP:WI}} & \opt{INT:W1} & - & - & - \\
    \hhline{~----}
    & \opt{HY1:W3} & -0.2827 & [-6.5, 5.9] & 0.928 \\
    \hhline{~----}
    & \opt{HY2:W3} & 0.4882 & [-5.6, 6.6] & 0.877 \\
     \hhline{~----}
    & \opt{POL:W3} & 1.8668 & [-4.3, 8.0] & 0.554 \\
     \hhline{~----}
    & \opt{HY1:W10} & 1.9846 & [-4.2, 16.6] & 0.529 \\
     \hhline{~----}
     & \cellcolor{green}\opt{HY2:W10} & \cellcolor{green}10.4442 & \cellcolor{green}[4.2, 16.6] & \cellcolor{green}$<$0.001 \\
     \hhline{~----}
     & \cellcolor{green}\opt{POL:W10} & \cellcolor{green}17.6876 & \cellcolor{green}[11.5, 23.8] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{4}{*}{\opt{DP:CL}} & \opt{INT:FD} & - & - & - \\
    \hhline{~----}
    & \opt{HY1:ARRAY} & -2.1297 & [-7.1,2.9] & 0.408 \\
    \hhline{~----}
    & \cellcolor{green}\opt{HY2:ARRAY} & \cellcolor{green}-12.3116 & \cellcolor{green}[-17.3,-7.2] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{POL:ARRAY} & \cellcolor{green}-13.6298 & \cellcolor{green}[-18.6,-8.5] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{5}{*}{\opt{CS:OR}} & \opt{CI:CLAS} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{1CFA:ALLO} & \cellcolor{green}27.5132 & \cellcolor{green}[22.1,32.8] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1TYP:ALLO} & \cellcolor{green}17.1402 & \cellcolor{green}[11.7,22.4] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \opt{1CFA:SMUS} & -5.2482 & [-10.6,0.1] & 0.054 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1TYP:SMUS} & \cellcolor{green}-11.0730 & \cellcolor{green}[-16.4,-5.7] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{5}{*}{\opt{CS:WI}} & \opt{CI:W1} & - & - & - \\
    \hhline{~----}
    & \opt{1CFA:W3} & 0.9160 & [-4.4,6.2] & 0.737 \\
    \hhline{~----}
    & \opt{1TYP:W3} & 2.2364 & [-3.1,7.5] & 0.413 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1CFA:W10} & \cellcolor{green}9.6493 & \cellcolor{green}[4.2,15.0] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1TYP:W10} & \cellcolor{green}17.3549 & \cellcolor{green}[11.9,22.7] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{3}{*}{\opt{CS:CL}} & \opt{CI:FD} & - & - & - \\
    \hhline{~----}
    & \opt{1CFA:ARRAY} & -2.2854 & [-6.6,2.0] & 0.305 \\
    \hhline{~----}
    & \cellcolor{green}\opt{1TYP:ARRAY} & \cellcolor{green}-8.1502 & \cellcolor{green}[-12.5,-3.7] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{5}{*}{\opt{OR:WI}} & \opt{CLAS:W1} & - & - & - \\
    \hhline{~----}
    & \opt{ALLO:W3} & 1.0841 & [-4.2,6.4] & 0.691 \\
    \hhline{~----}
    & \opt{SMUS:W3} & -0.3002 & [-5.6,5.0] & 0.912 \\
    \hhline{~----}
    & \opt{ALLO:W10} & 4.3739 & [-0.9,9.7] & 0.109 \\
    \hhline{~----}
    & \cellcolor{green}\opt{SMUS:W10} & \cellcolor{green}-5.4235 & \cellcolor{green}[-10.7,-0.1] & \cellcolor{green}0.047 \\
    \hline

    \multirow{3}{*}{\opt{OR:CL}} & \opt{CLAS:FD} & - & - & - \\
    \hhline{~----}
    & \cellcolor{green}\opt{ALLO:ARRAY} & \cellcolor{green}16.2518 & \cellcolor{green}[11.8,20.6] & \cellcolor{green}$<$0.001 \\
    \hhline{~----}
    & \cellcolor{green}\opt{SMUS:ARRAY} & \cellcolor{green}25.2598 & \cellcolor{green}[20.8,29.6] & \cellcolor{green}$<$0.001 \\
    \hline

    \multirow{3}{*}{\opt{WI:CL}} & \opt{W1:FD} & - & - & - \\
    \hhline{~----}
    & \opt{W3:ARRAY} & -0.3795 & [-4.7,3.9] & 0.864 \\
    \hhline{~----}
    & \cellcolor{green}\opt{W10:ARRAY} & \cellcolor{green}-5.2744 & \cellcolor{green}[-9.6,-0.9] & \cellcolor{green}0.018 \\
    \hline

  \end{tabular}
\end{tabular}
\caption{\textmd{Tradeoff for \aarray{} and \afield{}. Positive values
    in Est. column indicate a better tradeoff. R$^2$ of 0.75.}}
\hrule
\vspace{-12pt}
\label{tab:tradeoff}
\end{table*}

Next, we examine how analysis settings affect the tradeoff between
precision and performance, i.e., whether it is worthwhile to run a
slower analysis given that it may discharge more checks. We measure
this tradeoff using \emph{checks-per-minute (cpm)}
as a metric. We compute cpm by dividing the number of checks discharged by the overall analysis time.  For example, if an analysis discharged 20 checks and took
5 minutes, it would have a tradeoff of 4cpm. Of
course, this metric is only a rough approximation of the tradeoff an
analysis user might consider, but we believe it still gives us a useful,
quantitative way to compare analysis configurations. Also note that if
when run on a particular program a configuration could not finish its
analysis within the time budget, its cpm is 0 for that program.

Table~\ref{tab:tradeoff} summarizes a model of how
option settings affect a configuration's cpm. As in
Section~\ref{sec:precision}, we include the program and the
analysis options as independent variables, and we omit the program from the table.
 Overall we can see that the number of interactions in
this model is significantly more than the previous regressions,
suggesting that the relationship between analysis configuration and
cpm is very complex. Nonetheless, we can observe several results which
generally confirm the tradeoffs uncovered in the prior discussion.

\emph{Polyhedral analysis has a much worse overall tradeoff than other
  numeric domains, particularly for \opt{TD}.} The largest cpm
decrease over the interval domain 
for any individual setting is 48.6 from the polyhedral domain
(\opt{POL}). This result is expected given the significant performance
issues of \opt{POL} reported in Table
\ref{table:performance}. \opt{HY1} is similar to \opt{INT} in terms of
the tradeoff. However, the results of \opt{HY2} are more subtle. Although
\opt{HY2} still decreases cpm by 24.4 relative to the interval domain,
it is statistically better than \opt{POL} (notice the confidence
intervals do not overlap).
Moreover, \opt{HY2}'s interactions with \opt{BU},
\opt{1CFA}, \opt{1TYP}, and \opt{W10} all show improvements to cpm.


\emph{Bottom-up analysis generally has higher cpm than top-down
  variants.}  Bottom-up analysis (\opt{BU}) adds 28 cpm over the
baseline, and loses little when moving to relational domains:
\opt{HY2} subtracts 24.3 but \opt{BU:HY2} adds 10.5, while \opt{POL}
subtracts 48.6 but \opt{BU:POL} adds 17.8. Tradeoff \opt{BU:HY1} does
better still. These trends suggest that the efficiency of bottom-up
analysis outweighs its precision loss in terms of cpm. However, the
\opt{BU:ALLO} interaction shows bottom-up, allocation-based analysis
produces 24.1 fewer cpm (i.e., the individual effect of \opt{BU},
28.4, plus the interaction, -52.5) than top-down, allocation-site
based analysis. This result is also reflected in Table
\ref{table:performance}, because the performance of bottom-up,
allocation-based analysis is poor.

\emph{\opt{SMUS} has the best tradeoff among object representation
  settings.}  \opt{SMUS}, whose precision is similar to \opt{ALLO} in
Table~\ref{tab:precision}, and whose performance is close to
\opt{CLAS} in Table~\ref{table:performance}, outperforms both
\opt{CLAS} and \opt{ALLO} by about 13 cpm.

\emph{Other, more precise settings benefit from 1-CFA and
  type-sensitive analysis.}  In general, context sensitivity has
a negative impact on cpm compared to context-insensitive analysis,
especially for type-sensitive analysis. The decrease in cpm is 32.6
for type-based analysis (\opt{1TYP}) and 17.6 for
\opt{1CFA}. However, we note that context-sensitive analysis
benefits from the interactions with various other, more precise
settings, including allocation-based representation
(\opt{\{1TYP,1CFA\}:\{SMUS, ALLO\}}) and with delayed widening
(\opt{\{1TYP,1CFA\}:\{W3,X10\}}).
\begin{table*}[t!]
%\nocaptionrule
\small
\centering
\begin{tabular}{|c|r|r||r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
& \#  & \#  & \multicolumn{3}{c|}{\bf Best Performance} & \multicolumn{3}{c|}{\bf Best Precision} & \multicolumn{3}{c|}{\bf Best Precision (all term.)} & \multicolumn{3}{c|}{\bf Best Tradeoff}\\
\textbf{Name} & {\footnotesize \aarray{}} & {\footnotesize \afield{}} & \multicolumn{3}{c|}{{\footnotesize\opt{BU-INT-CI-CLAS-W1}}} & \multicolumn{3}{c|}{\opt{}} & \multicolumn{3}{c|}{{\footnotesize\opt{TD-HY2-1CFA-ALLO-W3}}} & \multicolumn{3}{c|}{{\footnotesize\opt{BU-HY1-CI-SMUS-W3}}}\\
\hline \hline
& & & Time & \aarray{} & \afield{} & Time & \aarray{} & \afield{} & Time & \aarray{} & \afield{} & Time & \aarray{} & \afield{}\\
\hline
 %\multirow{2}{*}{\opt{eclipse}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{TD:POL:1CFA:ALLO:W10}} &  &  & &  &  &  \\
eclipse & 367 & 280 & 1.14 & 35\% & 43\% & 14.64$^1$ & 82\% & 70\% & 3.13 & 78\% & 64\% & 1.04 & 71\% & 43\% \\
\hline
% \multirow{2}{*}{\opt{fop}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
fop & 552 & 537 & 3.70 & 34\% & 52\% & 15.93$^2$ & 80\% & 75\% & 15.93 & 80\% & 75\% & 8.14 & 64\% & 53\% \\
\hline
% \multirow{2}{*}{\opt{hsqldb}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
hsqldb & 364 & 301 & 4.24 & 39\% & 42\% & 118.88$^3$ & 79\% & 70\% & 118.88 & 79\% & 70\% & 5.72 & 75\% & 42\% \\
\hline
% \multirow{2}{*}{\opt{lusearch}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
lusearch & 372 & 302 & 0.94 & 35\% & 44\% & 17.04$^4$ & 81\% & 72\% & 3.27 & 77\% & 63\% & 1.18 & 74\% & 44\% \\
\hline
%\multirow{2}{*}{\opt{xalan}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
xalan & 371 & 299 & 0.85 & 39\% & 44\% & 13.92$^5$ & 80\% & 70\% & 3.61 & 78\% & 64\% & 1.12 & 74\% & 44\% \\

% eclipse & 367 & 280 & 1.14 & 35.1\% & 42.5\% & 14.64$^1$ & 81.5\% & 69.6\% & 3.13 & 77.9\% & 63.6\% & 1.04 & 70.6\% & 42.9\% \\
% \hline
% % \multirow{2}{*}{\opt{fop}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
% fop & 552 & 537 & 3.70 & 33.9\% & 52.1\% & 15.93$^2$ & 79.7\% & 74.7\% & 15.93 & 79.7\% & 74.7\% & 8.14 & 64.1\% & 52.7\% \\
% \hline
% % \multirow{2}{*}{\opt{hsqldb}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
% hsqldb & 364 & 301 & 4.24 & 39.3\% & 41.5\% & 118.88$^3$ & 78.6\% & 70.1\% & 118.88 & 78.6\% & 70.1\% & 5.72 & 74.7\% & 41.9\% \\
% \hline
% % \multirow{2}{*}{\opt{lusearch}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
% lusearch & 372 & 302 & 0.94 & 34.7\% & 44.0\% & 17.04$^4$ & 80.6\% & 72.2\% & 3.27 & 77.4\% & 62.6\% & 1.18 & 73.7\% & 44.4\% \\
% \hline
% %\multirow{2}{*}{\opt{xalan}} &  &  &  &  &  & \multicolumn{3}{c|}{\opt{}} &  &  & &  &  &  \\
% xalan & 371 & 299 & 0.85 & 38.8\% & 43.8\% & 13.92$^5$ & 80.1\% & 70.2\% & 3.61 & 77.9\% & 64.2\% & 1.12 & 73.6\% & 44.1\% \\


\hline
\end{tabular}
{\scriptsize $~^1$~\opt{TD-POL-1CFA-ALLO-W10} \hspace{.1cm}  $~^2$~\opt{TD-HY2-1CFA-ALLO-W3} \hspace{.1cm}  $~^3$~\opt{TD-HY2-1CFA-ALLO-W3} \hspace{.1cm} $~^4$~\opt{BU-POL-1CFA-ALLO-W10} \hspace{.1cm}  $~^5$~\opt{TD-POL-1CFA-ALLO-W10}}
\caption{Performance and precision for a range of analysis configurations.}
\vspace{-12pt}
\label{tab:rq4}
\end{table*}
 
\emph{\opt{W10} negatively affects the tradeoff.} Overall, \opt{W10}
decreases cpm by 35 over \opt{W1}, the second highest decrease for any
individual option setting after \opt{POL}. Because \opt{W10} is slow
in Table~\ref{table:performance} and insignificant for precision in
Table~\ref{tab:precision}, this result is expected.

\emph{\aarray{} and \afield{} have different tradeoffs.} There are
several significant interactions involving the analysis client,
notably \opt{ALLO:ARRAY} and \opt{SMUS:ARRAY}. Similarly to the
discussion in Section \ref{sec:precision}, this indicates that the impact
of analysis settings on two analysis clients are different.

\dropcomment{
\begin{table*}[th!]
%\nocaptionrule
\small
\centering
\begin{tabular}{|c|c||c|c|c||c|c|c|}
\hline
\multicolumn{2}{|c|}{} & \multicolumn{3}{c|}{${\tt T1\_A_1}$} & \multicolumn{3}{c|}{${\tt T2\_A_1}$} \\
\hline
{\bf Option} & {\bf Setting} & {\bf Est. (${\tt T1\_A_1}$)} & {\bf CI} & {\bf $p$-value} & {\bf Est. (${\tt T2\_A_2}$)} & {\bf CI} & {\bf $p$-value} \\
\hline
\multirow{2}{*}{\opt{AO}} & \opt{TD} & -& - & - & -& - & -\\
\hhline{~-------}
 & \opt{BU} & \cellcolor{green}32.2 &\cellcolor{green}[23.9, 40.5] & \cellcolor{green}$<$0.001 & 26.8 & [-1.5, 55.1] & 0.064\\
\hline
\multirow{4}{*}{\opt{DP}} & \opt{INT} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{POL} & \cellcolor{green}-58.5 & \cellcolor{green}[-70.2, -46.8] & \cellcolor{green}$<$0.001 & \cellcolor{green}-113.4 & \cellcolor{green}[-141.8, -85.1] & \cellcolor{green}$<$0.001\\
\hhline{~-------}
 & \opt{HY1} & -4.6 & [-16.3, 7.1] & 0.440 & -1.1 & [-29.4, 27.2] & 0.938\\
\hhline{~-------}
 & \opt{HY2} & \cellcolor{green}-34.8 & \cellcolor{green}[-46.5, -23.1] & \cellcolor{green}$<$0.001 & 21.0 & [-7.3, 49.3] & 0.147\\
 \hline
 \multirow{3}{*}{\opt{CS}} & \opt{CI} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{1CFA} & \cellcolor{Gray}-17.1 & \cellcolor{Gray}[-27.8, -6.3] & \cellcolor{Gray}0.002 & -3.1 & [-27.6, 21.5] & 0.807\\
\hhline{~-------}
 & \opt{1TYP} & \cellcolor{Gray}-36.0 & \cellcolor{Gray}[-46.8, -25.3] & \cellcolor{Gray}$<$0.001 & 22.3 & [-2.2, 46.8] & 0.075 \\
 \hline
\multirow{3}{*}{\opt{OR}} & \opt{CLAS} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{SMUS} & \cellcolor{green}50.7 & \cellcolor{green}[40.0, 61.4] & \cellcolor{green}$<$0.001 & \cellcolor{green}162.3 & \cellcolor{green}[129.9, 194.8] & \cellcolor{green}$<$0.001\\
\hhline{~-------}
 & \opt{ALLO} & \cellcolor{green}26.8 & \cellcolor{green}[16.1, 37.6] & \cellcolor{green}$<$0.001 & \cellcolor{green}179.8 & \cellcolor{green}[147.4, 212.3] & \cellcolor{green}$<$0.001\\
 \hline
 \multirow{3}{*}{\opt{WI}} & \opt{W1} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{W3} & -3.3 & [-13.4, 6.8] & 0.522 & 0.1 & [-12.2, 12.3] & 0.991\\
\hhline{~-------}
 &\opt{W10} & \cellcolor{green}-37.9 & \cellcolor{green}[-48.0, -27.7] & \cellcolor{green}$<$0.001 & -11.8 & [-24.1, 0.5] & 0.059\\
 \hline
 \hline
  \multirow{4}{*}{\opt{AO:DP}} & \opt{TD:INT} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{BU:POL} & \cellcolor{green}15.0 & \cellcolor{green}[6.8, 23.3] & \cellcolor{green}$<$0.001 & \cellcolor{green}116.1 & \cellcolor{green}[87.8, 144.5] & \cellcolor{green}$<$0.001\\
\hhline{~-------}
 & \opt{BU:HY1} & 6.6 & [-1.7, 14.8] & 0.119 & 3.0 & [-25.3, 31.3] & 0.834\\
\hhline{~-------}
 & \opt{BU:HY2} & 5.9 & [-2.4, 14.2] & 0.162 & -14.3 & [-42.6, 14.1] & 0.324\\
 \hline
 \multirow{3}{*}{\opt{AO:CS}} & \opt{TD:CI} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{BU:1CFA} & \cellcolor{green}-23.8 &  \cellcolor{green}[-31.0, -16.7] & \cellcolor{green}$<$0.001 & -1.0 &  [-25.5, 23.5] & 0.936\\
\hhline{~-------}
 & \opt{BU:1TYP} & \cellcolor{green}-29.2 & \cellcolor{green}[-36.4, -22.1] & \cellcolor{green}$<$0.001 & \cellcolor{green}-55.2 & \cellcolor{green}[-79.7, -30.7] & \cellcolor{green}$<$0.001 \\
 \hline
 \multirow{3}{*}{\opt{AO:OR}} & \opt{TD:CLAS} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{BU:SMUS} & 4.3 & [-2.9, 11.4] & 0.244 & \cellcolor{green}-31.0 & \cellcolor{green}[-55.6, -6.5] & \cellcolor{green}0.013\\
\hhline{~-------}
 & \opt{BU:ALLO} & \cellcolor{green}-58.0 & \cellcolor{green}[-137.1, -88.0] & \cellcolor{green}$<$0.001 & \cellcolor{green}-112.5 & \cellcolor{green}[-65.1, -50.8] & \cellcolor{green}$<$0.001\\
 \hline
  \dropcomment{
 \multirow{7}{*}{\opt{DP:CS}} & \opt{INT:CI} & - & - & - & X & X & X\\
\hhline{~-------}
 & \opt{POL:1CFA} & 7.3 & [-2.8, 17.4] & 0.157 & X & X & X\\
\hhline{~-------}
 & \opt{POL:1TYP} & \cellcolor{Gray}29.1 & \cellcolor{Gray}[19.0, 39.2] & \cellcolor{Gray}$<$0.001 & X & X & X \\
\hhline{~-------}
 & \opt{HY1:1CFA} & 1.0 & [-9.2, 11.1] & 0.853 & X & X & X\\
\hhline{~-------}
 & \opt{HY1:1TYP} & 3.4 & [-6.7, 13.5] & 0.513 & X & X & X\\
\hhline{~-------}
 & \opt{HY2:1CFA} & \cellcolor{Gray}10.8 & \cellcolor{Gray}[0.7, 21.0] & \cellcolor{Gray}0.036 & X & X & X\\
\hhline{~-------}
 & \opt{HY2:1TYP} & \cellcolor{Gray}20.8 & \cellcolor{Gray}[10.6, 30.9] & \cellcolor{Gray}$<$0.001& X & X & X \\
 \hline
 \multirow{7}{*}{\opt{DP:OR}} & \opt{INT:CI} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{POL:SMUS} & \cellcolor{green}-20.4 & \cellcolor{green}[-30.5, -10.2] & \cellcolor{green}$<$0.001 & \cellcolor{green}-84.5 & \cellcolor{green}[-119.2, -49.8] & \cellcolor{green}$<$0.001 \\
\hhline{~-------}
 & \opt{POL:ALLO} & -8.4 & [-18.5, 1.7] & 0.103 & \cellcolor{green}-71.2 & \cellcolor{green}[-105.9, -36.5] & \cellcolor{green}$<$0.001\\
\hhline{~-------}
 & \opt{HY1:SMUS} & -5.4 & [-15.5, 4.7] & 0.295 & 0.1 & [-34.6, 34.8] & 0.994\\
\hhline{~-------}
 & \opt{HY1:ALLO} & -9.2 & [-19.3, 0.9] & 0.075 & 4.0 & [-30.7, 38.7] & 0.821\\
\hhline{~-------}
 & \opt{HY2:SMUS} & \cellcolor{green}-20.1 & \cellcolor{green}[-84.4, -15.1] & \cellcolor{green}$<$0.001 & \cellcolor{green}-49.8 & \cellcolor{green}[-30.3, -10.0] & \cellcolor{green}0.005\\
\hhline{~-------}
 & \opt{HY2:ALLO} & -8.3 & [-18.5, 1.8] & 0.106 & \cellcolor{green}-39.5 & \cellcolor{green}[-74.2, -4.8] & \cellcolor{green}0.026\\
 \hline
 \multirow{7}{*}{\opt{DP:WI}} & \opt{INT:W1} & - & - & - \\
\hhline{~-------}
 & \opt{POL:W3} & 2.3 & [-7.8, 12.4] & 0.656 \\
\hhline{~-------}
 & \opt{POL:W10} & \cellcolor{green}21.2 & \cellcolor{green}[11.1, 31.3] & \cellcolor{green}$<$0.001 \\
\hhline{~-------}
 & \opt{HY1:W3} & -0.4 & [-10.5, 9.7] & 0.941 \\
\hhline{~-------}
 & \opt{HY1:W10} & 2.6 & [-7.5, 12.7] & 0.613 \\
\hhline{~-------}
 & \opt{HY2:W3} & 0.8 & [-9.3, 11.0] & 0.869 \\
\hhline{~-------}
 & \opt{HY2:S10} & \cellcolor{green}13.9 & \cellcolor{green}[3.8, 24.1] & \cellcolor{green}0.007 \\
 \hline
 }
 \multirow{5}{*}{\opt{CS:OR}} & \opt{CI:CLAS} & - & - & - & - & - & -\\
\hhline{~-------}
 & \opt{1CFA:SMUS} & \cellcolor{Gray}-14.5 & \cellcolor{Gray}[-23.3, -5.7] & \cellcolor{Gray}0.001 & -0.1 & [-30.1, 30.0] & 0.997\\
\hhline{~-------}
 & \opt{1TYP:SMUS} & \cellcolor{Gray}-25.6 & \cellcolor{Gray}[-34.4, -16.8] & \cellcolor{Gray}$<$0.001 & -6.8 & [-36.8, 23.2] & 0.657\\
\hhline{~-------}
 & \opt{1CFA:ALLO} & \cellcolor{green}26.7 & \cellcolor{green}[18.0, 35.5] & \cellcolor{green}$<$0.001 & 21.9 & [-8.2, 51.9] & 0.153\\
\hhline{~-------}
  & \opt{1TYP:ALLO} & \cellcolor{Gray}10.0 & \cellcolor{Gray}[1.2, 18.8] & \cellcolor{Gray}0.025 & \cellcolor{green}-77.8 & \cellcolor{green}[-107.8, -47.7] & \cellcolor{green}$<$0.001\\
 \hline
 \dropcomment{
  \multirow{5}{*}{\opt{CS:WI}} & \opt{CI:W1} & - & - & - \\
\hhline{~-------}
 & \opt{1CFA:W3} & 0.9 & [-7.8, 9.7] & 0.833 \\
\hhline{~-------}
 & \opt{1TYP:W3} & 2.5 & [-6.3, 11.3] & 0.574 \\
\hhline{~-------}
 & \opt{1CFA:W10} & \cellcolor{green}10.5 & \cellcolor{green}[1.7, 19.3] & \cellcolor{green}0.019 \\
\hhline{~-------}
  & \opt{1TYP:W10} & \cellcolor{green}19.6 & \cellcolor{green}[10.8, 28.4] & \cellcolor{green}$<$0.001 \\
 \hline
   \multirow{5}{*}{\opt{OR:WI}} & \opt{CI:W1} & - & - & - \\
\hhline{~-------}
 & \opt{SMUS:W3} & -0.84 & [-9.6, 7.9] & 0.850 \\
\hhline{~-------}
 & \opt{ALLO:W3} & 0.85 & [-7.9, 9.6] & 0.849 \\
\hhline{~-------}
 & \opt{SMUS:W10} & \cellcolor{green}-13.2 & \cellcolor{green}[-21.9, -4.4] & \cellcolor{green}0.003 \\
\hhline{~-------}
  & \opt{ALLO:W10} & -0.6 & [-9.3, 8.2] & 0.900 \\
 \hline
 }
\end{tabular}

%\jeff{Indicate in caption whether positive or negative values are good.}
\caption{\textmd{\afield{} performance and precision tradeoffs. Positive values in Est. columns indicate better tradeoffs.}}
\vspace{-12pt}
\label{table:A1tradeoff}
\end{table*}
}

\subsection{RQ4: Overall quality}
\label{pimpact}

Finally, we examine how well ``best'' analysis configurations
work for \aarray{} and \afield{}, in absolute terms. We chose
configurations by examining the regressions in
Tables~\ref{table:performance}, \ref{tab:precision},
and~\ref{tab:tradeoff} and picking the best option settings
for each (details below).

Table~\ref{tab:rq4} shows the results. The first three columns list
each benchmark and its total number of array accesses and numerically
typed field reads. Then for each best analysis (in various terms), the
remaining column groups show that analysis' running time and the
percent of array accesses checked and numerically typed field reads
that were constrained.

We chose the best analyses as follows. For performance, we examined 
Table~\ref{table:performance} and found \opt{BU} is the statistically
best analysis order. Any choice for domain except \opt{POL} is
equivalent; we choose \opt{INT} because it is the simplest. Similarly,
we choose \opt{CI} and \opt{CLAS} because those are the simplest of a
statistically equivalent set of choices. And we choose \opt{W1}
because it is statistically better than \opt{W10} and simpler.

For Table~\ref{tab:precision}, recall the regression omitted analysis
configurations that timed out---hence the best configuration according
to that regression might not, and in fact does not, complete on all
the benchmarks. Thus, we show two results for precision. The first
group of precision results is based on the most precise
configuration for each benchmark  individually. The next group picks
one overall configuration for which all benchmarks complete, and which
is close to the best configuration in Table~\ref{tab:precision}. For
example, for domain, instead of \opt{POL}, which times out on some
programs, we use \opt{HY2}, which is a close second in the table. Note
that the precision table did not specify a setting for object
representation or widening (they were not needed to fit the data); we
chose \opt{1CFA} and \opt{W3} because those are the most precise
variants for which all programs complete.

Finally, we picked the best tradeoff from Table~\ref{tab:tradeoff}. In
that table, \opt{BU}, \opt{CI}, and \opt{SMUS} are statistically the
best. We chose \opt{HY1} as it does best when combined with \opt{BU}
and \opt{W3} is faster with the same precision as \opt{W10}.

Looking over the results, we make several observations. First, the
best performing configuration is far faster than the most precise
configurations. However, the running time is not much better than the
best tradeoff configuration. Moreover, for \aarray{}, the best
tradeoff configuration is almost as precise as the best precision
configuration, showing that for \aarray{} it is possible to achieve
both good precision and good performance. The story is less good for
\afield{}, where precision for the best tradeoff drops considerably
compared to the most precise analyses. This is because \opt{HY1} is
far less precise than \opt{HY2} or \opt{POL}. Indeed, if we used
\opt{HY2} instead, we would have far better results, but \opt{fop}'s
analysis no longer terminates.\footnote{In particular: \opt{eclipse}
  2.18m, 75\%, 60\%; \opt{hsqldb} 8.99m, 76\%, 63\%; \opt{lusearch}
  1.88m, 75\%, 65\%; \opt{xalan} 2.04m, 75\%, 62\%.}

Second, we see that the best terminating configuration for each
program individually always utilizes \opt{ALLO}, \opt{1CFA}, and
\opt{HY2} (or \opt{POL}); in all cases but \opt{lusearch} it uses
\opt{TD} because \opt{BU} is more expensive and may not terminate. 

Third, we see that the best precision configuration that terminates on
all programs has precision close to the individual best configurations
(but moreso for \aarray{} than for \afield{}). This suggests that if a user is
most interested in high precision, it may not be necessary to
customize the analysis for a particular subject program.

Finally, bottom-up analysis provides a good tradeoff for \aarray{},
and context-insensitive points-to analysis is sufficient. As mentioned
earlier, we believe this is due to the nature of the client: array
bounds checking likely performs a lot of local reasoning, and the
analysis provides a sufficient amount of ``pseudo'' context
sensitivity, as discussed in Section~\ref{sec:precision}.

